Tensor Networks: Phase transition phenomena on hyperbolic and fractal geometries

One of the challenging problems in the condensed matter physics is to understand the quantum many-body systems, especially, their physical mechanisms behind. Since there are only a few complete analytical solutions of these systems, several numerical simulation methods have been proposed in recent years. Amongst all of them, the Tensor Network algorithms have become increasingly popular in recent years, especially for their adaptability to simulate strongly correlated systems. The current work focuses on the generalization of such Tensor-Network-based algorithms, which are sufficiently robust to describe critical phenomena and phase transitions of multistate spin Hamiltonians in the thermodynamic limit. We have chosen two algorithms: the Corner Transfer Matrix Renormalization Group and the Higher-Order Tensor Renormalization Group. This work, based on tensor-network analysis, opens doors for the understanding of phase transition and entanglement of the interacting systems on the non-Euclidean geometries. We focus on three main topics: A new thermodynamic model of social influence, free energy is analyzed to classify the phase transitions on an infinite set of the negatively curved geometries where a relation between the free energy and the Gaussian radius of the curvature is conjectured, a unique tensor-based algorithm is proposed to study the phase transition on fractal structures.

==> Social1.tex <==
\section{Models of social behavior} \label{chap4}

%\subsection{Introduction}

The last couple of years has witnessed an increasing interest in the study of the collective behavior of social systems. Social systems are composed of people (individuals) who interact with one another. These interactions influence the people engaged in them, and after many interactions, global properties emerge, i.e., a macro-level behavior of groups or whole societies. An essential question is how these microscopic (local) interactions lead to the global macroscopic (global) properties of the system under investigation. This question can be also answered by tools of the statistical physics. The approach of the statistical physics is used extensively in the study of collective phenomena. 

One may then ask, ``{\it Statistical physics is used for study of interacting particles, aren't humans astonishingly much more complicated?}" This is a reasonable objection. Inevitably, every modeling of social agents may imply severe simplifications of the reality. The social agents are modeled by a rather limited set of variables which represent their properties or states. The microscopic interaction among the agents should be 
%%% Jozef: typo - "this" -> "thus" 
thus
%%% 
defined sensibly and realistically to capture the dynamics of the social behavior, which is not a trivial task. However, the concept known from the statistical physics as {\it universality} says that the large-scale phenomena do not depend on the microscopic details of the process. They depend only on 
%%% Jozef: insert hyphen - "higher level" -> "higher-level"
higher-level
%%%
features, like symmetries, dimensions or conservation laws. Keeping this fact in mind, one can learn something about a system just by reproducing the most important properties of the elements and their interactions. 

Studying social dynamics is a rapidly evolving area of scientific studies. It has its applications in disciplines as diverse as sociology, economics, political science, and anthropology. It is a 
%%% Jozef: overused word: remove "really"
hard task to present the state-of-art in this subject. However, we have
%%% Jozef: two times "however"- , however, 
found a very useful work in this area~\cite{Castellano_over}. Other resources will be referred to later on. 

Major regularities can emerge spontaneously in social systems, as it is frequently observable in the real world. This can be understood as an order-disorder transition. Among examples of such transitions, we count the spontaneous formation of common language/culture or the emergence of consensus on an issue, collective motion, a hierarchy. The drive toward the ordering is the tendency of agents to become alike as they interact. The term for this mechanism is \textit{social influence}. It is analogous to ferromagnetic interaction in magnetic materials. The Ising model, briefly introduced in Subsection~\ref{Ising_model_subs}, is a model of such a ferromagnetic material. It can, however, be considered as a very simple model of opinion dynamics, wherein the agents are influenced by the state of the majority of their nearest neighbors. 

One way of considering the unknown influence, or some hidden details of the social dynamics, is to introduce the {\it noise}, which corresponds to a variability in the states of the agents. A natural question arises, ``{\it Does the presence of a noise hinder the ordered state?}"
The role of noise in one particular model (the Axelrod model) is to be discussed. 

Traditionally, the statistical physics deals with regular systems such as lattices, where the elements are located on the sites and usually interact with the nearest neighbors only or involve all-to-all interactions (the mean-field approximation). However, social interactions exhibit the interaction pattern which is denoted as complex networks. The role of topology is a highly studied topic in this context; nonetheless, our work is not concerned about it. 

The simplest model of the opinion formation is the Voter model. Each agent $s_i$ in this model is endowed with a binary variable $s_i = \pm 1$. This variable represents, e.g., the answer to the yes-no question. The interaction is defined by the following algorithm: First one randomly selects an agent $i$, chooses one of the neighbors $j$ at random, and then changes the opinion of agent $s_i$ to be equal to the opinion of a selected neighbor $s_j$. This process mimics the homogenization of opinions; however, the convergence to a uniform state cannot be always guaranteed, because the interactions are random and only between two agents at each step. For $D$-dimensional lattice, the described mechanism leads to slow coarse-graining processes, where spatially ordered regions grow, i.e., large regions tend to expand and ``consume" the small ones. 

%%% Jozef: explanation - there are several problems with the caption of the figure \ref{Voter}, the description is not correct! (my fault)  
%%% I think this figure can be omitted as it doesn't add anything to the text - everything is already clear from the main text 
%%% , cf. Fig.~\ref{Voter}. 

\iffalse 
%%% Jozef: This picture is removed 
\begin{figure}[tb]
\centering
 \includegraphics[width=\textwidth]{Voter.pdf}
     \caption{The evolution of the Voter model for agents located on the sites of the
two-dimensional square lattice $200\times200$. The black dots represent opinions $+1$,
while the empty spaces represent opinions $-1$. From left to right: Starting from a
disordered configuration, as captured at times $t=5, 50, 500, 1000$ (after~\cite{Dornic}).}
\label{Voter}
 \end{figure}  
 \fi 

The evolution of the system can be described by the density of active interfaces between ordered regions $n_a$. The following scaling of evolution of Voter model was found in~\cite{Krapivsky},
\begin{equation} 
n_a(t) \sim \begin{cases}
    t^{-(2-d)/2},  & D<2\text{,}\\
    1/\ln(t),          & D=2\text{,}\\
    a - bt^{-d/2}, & D>2\text{.} 
  \end{cases}
\end{equation}
Amongst some other models of the opinion formation belong: A majority rule model, models of social impact, Sznajd model, and bounded confidence models. For more details concerning the Voter model as well as the other models, see Refs.~\cite{Castellano_over,BBV}.

Besides the opinion dynamics, much interest has been focused on the related field of cultural dynamics. There is no sharp distinction between the two, however, in cultural dynamics, each agent is described by a vector of variables instead of a scalar variable as we have seen in the opinion dynamics. A paradigmatic model of the cultural dynamics is the Axelrod model which we focus on.

As it should be clearer from the text, our approach is to view the agents as being adaptive instead of being rational, in particular, with a focus on communication rather than strategy. The latter approach has, however, been studied extensively. Let us mention at least prisoner's dilemma, where the agents (players) interact (play) pairwise and have two strategies which they can choose, i.e., they can decide whether to cooperate or not. For more details, see the references in~\cite{BBV}. 

We summarize this brief introduction with a note about co-evolution of opinions and topology. So far, the topology of the network was considered to be fixed and served as a playground for a dynamical process. On the other hand, many real networks are of dynamical nature, i.e., the topology of such networks changes with time. The dynamical process taking place on the network can be coupled with the evolution of the topology. This is particularly relevant for social networks. One example is a link removal (or re-wiring) between two agents with dissimilar opinions and creation of new links between other two random agents, or with a preference between similar ones. There is a huge number of works concerning this topic, for survey, see Refs.~\cite{BBV,Castellano_over}.

\subsection{The Axelrod model}\label{AXM}

Axelrod proposed a simple, yet ambitious, model of cultural assimilation and diversity, which is based on two mechanisms: \textit{social influence} and \textit{homophily}~\cite{Axelrod}. The former means, that after interacting, people become more similar than before. In other words, communication reduces differences among the people. The latter is that the probability of social interaction depends on the similarity between two agents. It is based on the idea, that the more similar two people are, the easier their communication becomes. It might seem that this mechanism leads to the homogenization of society. However, it can generate a global polarization, where different cultures are allowed to coexist. The mechanism of this model might be relevant for such topics as state formation, succession conflicts, trans-national integration, or domestic cleavages.

Each agent has $f$ different cultural {\it features}, which we denote as $(\sigma_1, \sigma_2, \dots , \sigma_f)$, and each of the 
%%% Jozef: use plural - "feature" -> "features"
features can assume $q$ different values ({\it traits}), $\sigma_{\alpha} = 0, 1, ..., q-1$. It means that each agent can be in one of $q^f$ possible states. Each feature represents one of the cultural dimension such as, e.g., language, religion, technology, style of dress, and the like. Agents are placed on sites of a regular two-dimensional square lattice $L \times L$ and can interact only with the nearest neighbors (the longer ranged interactions are to be considered later). The dynamics runs in two steps as follows:
\begin{itemize}
\item[1]{An agent at site $i$ and one of his neighbors $j$ are selected randomly.}
\item[2]{The selected agents interact with the probability being proportional to the number of the features for which they share the same value,
\begin{equation}
\omega_{ij} = \frac{1}{f}\sum_{\alpha=1}^{f}\delta\left(\sigma_{\alpha}^{(i)}, \sigma_{\alpha}^{(j)}\right),
\end{equation}
where $\delta(\ast,\ast)$ is the Kronecker's delta.
The interaction consists of random selection of the feature the two agents differ, $\sigma_{\alpha}^{(i)} \neq \sigma_{\alpha}^{(j)}$ and consequently setting this feature of the neighbor to be equal to $\sigma_{\alpha}^{(i)}$. }
\end{itemize}
These two steps are repeated as long as needed. 

The described process can lead either to a global homogenization or to a fragmented state with coexistence of different homogeneous regions, as shown in Fig.~\ref{map}. As the two agents do interact, they share more specific cultural features. More features tend to be shared over a larger area and a cultural region (with all features being exactly the same) can be created. Eventually, the system may end in a state where no other change is possible. Those features of all neighbors are either identical or there is no match, as they do not interact at all. Several {\it stable regions} can be created. A question of interest is how many.  

%%% Jozef: I believe that this figure is OK - I have already rearranged it before 
\begin{figure}[tb]
\begin{center}
\begin{tabular}{cccc}
\includegraphics[width=.22\linewidth]{axel_map1.pdf} &
\includegraphics[width=.22\linewidth]{axel_map2.pdf} &
\includegraphics[width=.22\linewidth]{axel_map3.pdf} &
\includegraphics[width=.22\linewidth]{axel_map4.pdf} \\
$t=0$ &  $t=2\times10^4$ & $t=4\times10^4$ & $t=8\times10^4$
\end{tabular}
\end{center}
  \caption{Example of the four maps of the cultural similarities. Simulation was conducted for lattice size $10 \times 10$ only, the number of the features is $f = 5$, and the number of possible values of each feature is $q=10$. The cultural similarity (number of the shared features) between adjacent agents is coded as black for $\omega_{ij} \leq 20\%$, dark grey for $\omega_{ij}=40\%$, gray for $\omega_{ij}=60\%$, light grey for $\omega_{ij}=80\%$, and white for $\omega_{ij}=100\%$. The time evolution denotes the number of events $t$ (after~\cite{Axelrod}).}
  \label{map}
\end{figure}

As $f$ increases (with $q$ being fixed) the probability of sharing at least one of the features is higher. In that case, the average number of the stable regions (with respect to different runs) decreases. On the contrary, as $q$ increases (with $f$ being fixed) the probability of sharing at least one of the features is smaller and thus the average number of stable regions increases. 

The longer-ranged interactions have also been considered, i.e., the interactions between second nearest neighbors, third nearest neighbors, etc. It is intuitively clear that if the agents could interact over larger distances, the process of cultural convergence would have been made easier. The longer the interactions are allowed, the smaller is the average number of stable regions, as expected.

Another studied question was the dependence of the average number of stable regions on the size of the lattice (size of a territory). Axelrod provided some preliminary results which suggested that this number increases with size of the lattice for small lattices and after certain size it decreases. 
%%% Jozef: I suggest to remove this
%%% , see Fig.~\ref{territory}. 
Small lattices do not have enough space to contain many stable regions, thus it is understood this number would increase as the size of the lattice increases. However, it is surprising that the large lattices would have had fewer stable regions than moderately-sized lattices. 

\iffalse 
%%% Jozef: I don't find this figure interesting. All the information is already in the text: 
%%% "Axelrod provided some preliminary results which suggested that this number increases with size of the lattice for small lattices and after certain size it decreases"
\begin{figure}[tb]
\centering
 \includegraphics[width=3.7in]{territory.pdf}
     \caption{Dependence of the average number of stable regions on the size of the lattice $L \times L$. The results for $f=5$ and $q=15$ are averaged over 40 runs, except for the lattice sizes $50 \times 50$ and $100 \times 100$, where it was only 10 (after~\cite{Axelrod}).
}\label{territory}
 \end{figure}  
 \fi 
 
 \iffalse
 %%% Jozef: It is actualy a good figure, but any change would be too apparent and would just decrease its value
\begin{figure}[tb!h]
\centering
 \includegraphics[width=3.9in]{Axelrod_1.pdf}
     \caption{Behavior of the order parameter $\left<S_{\text{max}}\right>$ with respect to $q$ for the three different system sizes and $f=10$. The identical quantity is reported for $f=2$ in the inset (after~\cite{Castellano1}).
}\label{Axelrod_1}
 \end{figure}  
 \fi 

A detailed phase diagram of the model was studied in Ref.~\cite{Castellano1}. The order parameter was defined as the average size of the largest stable region $\left<S_{\text{max}}\right>$. For fixed $f$, there is a critical value $q_c$ such that $\left<S_{\text{max}}\right>$ increases with the linear system size $L$ and tends to $L^2$ for $q<q_c$, whereas $\left<S_{\text{max}}\right>/L^2 \rightarrow 0$ for $q>q_c$. For the two-dimensional lattices, nature of these phase transitions depends on the value of $f$. For $f=2$ the transition is continuous, whereas for $f>2$ it becomes discontinuous, see 
%%% Jozef: change to a reference to a specific figure from the cited article Fig.~\ref{Axelrod_1} 
Fig.~1 in Ref.~\cite{Castellano1}. 
For the one-dimensional systems, the transition remains continuous for all values of $f$~\cite{Klemmd}.

\iffalse
\begin{figure}[tb]
\centering
 \includegraphics[width=3.7in]{Noise.pdf}
  \caption{The universal scaling of the order parameter $\left<S_{\text{max}}\right>$ as a function of the effective noise rate $r' = r(1-1/q)$ for different values of $q$. The simulations have been run for systems with the size $50\times 50$ and $f=10$. (After \cite{Klemmc}.)
}\label{Noise}
 \end{figure}  
 \fi 

\textit{Cultural drift} can be modeled as a spontaneous change of a feature at certain rate $r$. The order-disorder transition induced by a noise was demonstrated in Ref.~\cite{Klemmc}. 
The transition depends on the value of $q$, which becomes weaker for larger values of $q$,
as plotted in Fig.~3 in Ref.~\cite{Klemmc}. 
%%% Jozef: this figure is not necessary to show 
%%% Fig.~\ref{Noise}.
At small noises, the system tends to homogeneity, because the disordered configurations are unstable with respect to the perturbations enhanced by the noise. On the contrary, when the noise rate gets larger, the system becomes heterogeneous, as domains disappear, which is compensated by creating new ones. 

The effect of the mass media can be modeled by interactions among the agents with a global (uniform) {\it field}. In Ref.~\cite{Gonzalez05}, the global field was introduced to represent the mass-media cultural message as a set of $f$ parameters, $M=(\mu_1, \mu_2, ..., \mu_f)$. A selected agent interacts with the field, as if it was an agent with probability $B$, and with one of his actual neighbors with probability $1-B$. Surprisingly, the global field favors the multi-cultural phase. In other words, $q_c$ is smaller with addition of the global field and depends on $B$. For $B$ larger than a certain threshold, such that $q_c(B)=0$, only the disordered phase is present. A global coupling and a local non-uniform coupling were considered in Ref.~\cite{Gonzalez}.

The social networks have a complex topology as we have mentioned above. With respect to this fact, the Axelrod model was considered on networks with complex topological characteristics. For Watts-Strogatz two-dimensional networks, the previously defined $q_c$, starts growing as the disorder parameter increases~\cite{Klemmb}. For random scale-free networks, $q_c$ diverges with the size of the system as $L^\beta$ (here, $\beta \sim 0.4$ for Barab\'{a}si-Albert type of networks), where $L$ is the size of the network~\cite{Klemmb}.

\subsection{Thermodynamic version of Axelrod model}\label{tAXM}

In Ref.~\cite{Gandica}, a thermodynamic version of the Axelrod model has been proposed. Let us remark that the original Axelrod model is th model out of equilibrium, i.e, it does not satisfy the equilibrial conditions, as detailed balance\footnote{
We assume that each node (agent) $i$ can be in one of the possible states, i.e., $\sigma_i = 0,1, 2, ..., q-1$. The knowledge of the state of all the nodes defines a microscopic state (microstate) $\sigma(t) = (\sigma_1(t), \sigma_2(t), \dots, \sigma_L(t))$, where $L$ is size of the network.
Dynamical description of the system is given by the master equation. The master equation is an evolution equation for probability $P(\sigma, t)$ of finding the system at time $t$ in a microstate $\sigma$. In continuous time approximation, the master equation is
\begin{equation*}
\partial_t P(\sigma, t) = \sum_{\sigma'} \left[P(\sigma', t)W(\sigma' \rightarrow \sigma) - P(\sigma, t) W(\sigma \rightarrow \sigma')\right],
\end{equation*}
where the terms $W(\sigma' \rightarrow \sigma)$ represent the transition rates from one microstate (configuration) to another. 
As we can see, the solution of the master equation provides only statistical information about the system evolution.

One of the interests is to find a stationary state of the system (if exists)
$\lim_{t \to +\infty} P(\sigma, t) = P_{\infty}(\sigma)$.
Stationary distribution for equilibrial physical systems is given by the well-known Boltzmann-Gibbs distribution
$P_{\infty}(\sigma) = P_{\text{eq}}(\sigma) = \exp[-{\cal H}(\sigma)/k_{\text{B}}T]/{\cal Z}$,
where ${\cal H}(\sigma)$ is a Hamiltonian of the system. The partition function ${\cal Z}$ provides the proper normalization 
$ {\cal Z} = \sum_{\sigma} \exp(-{\cal H}(\sigma)/k_{\text{B}}T) $ of the distribution.
The stationary distribution for the equilibrium system may be obtained by the system Hamiltonian and there is no need to solve the master equation. 

At equilibrium, each elementary process should be equilibrated by its reverse process. This is what the so-called {\it detailed balance condition} states
\begin{equation*}
P_{\text{eq}}(\sigma) W(\sigma \rightarrow \sigma') = P_{\text{eq}}(\sigma') W(\sigma' \rightarrow \sigma).
\end{equation*}
This condition gives zero contribution for each pair on the right-hand side of the master equation. 
The detailed balance is not necessarily fulfilled, i.e. $\partial_t P(t) =0$, and the non-equilibrium systems can also reach the stationary state, however, with more complicated cancellation relations in the master equation. Most of the real systems are actually non-equilibrial and we thus cannot use the equilibrium thermodynamic formulations.
} is violated. The Hamiltonian proposed by the authors is
%
\begin{equation} \label{Hamiltonian_A}
{\cal H} = - \sum_{\alpha=1}^{f} \left[ \sum_{\left<ij\right>}  J_{ij\,} \delta\left(\sigma_{i \alpha}^{~},\sigma_{j \alpha}^{~}\right) + h \sum_{i} \delta\left(\sigma_{i\alpha}^{~},h_{\alpha}^{~}\right) \right]
\end{equation}
%
with the interaction factor
\begin{equation}
J_{ij} = \sum_{\alpha'=1}^{f}J\delta\left(\sigma_{i\alpha'},\sigma_{j\alpha'}\right). 
\end{equation}
The index $\alpha$ denotes the features, the indices $i$ and $j$ label the lattice sites, where the agents are localized, and the cultural feature $\alpha$ of an agent $i$ can take $q$ values, $\sigma_{i\alpha} = 0, 1, 2, \dots, q-1$. Here, $h_{\alpha}$ is the magnetic field with $q$ values ($h_{\alpha} = 0, 1, 2, \dots, q-1$), $h$ is the magnitude of the field uniformly imposed. The meaning of the interaction factor $J_{ij}$ is such that it defines the number of shared features between two agents $i$ and $j$ multiplied by a constant $J$. 

The Hamiltonian (\ref{Hamiltonian_A}) is inspired by the Potts model, however, the interaction factor $J_{ij}$ depends on the global state of the $f$ variables $(\sigma_{i1}, \sigma_{i2}, \dots , \sigma_{if})$. The thermodynamic and the critical properties were calculated analytically in the one-dimensional case, where the order-disorder phase transition occurred at $T=0$ regardless of $f$ and $q$, as it is in agreement with the one-dimensional Potts (Ising) model~\cite{Baxter}. 

As we have mentioned earlier, the Axelrod model was also studied with the noise (which represents the cultural drift). It has been shown that for the noise rate $r<r_c$ the system converges to the monocultural state, whereas for $r>r_c$ the system converges to the multicultural state, where $r_c$ is a certain critical value of the noise rate and depends on the system size, not on $q$ \cite{Klemm2005, Klemmc, Toral}. In the one-dimensional case, $r_c$ scales as $r_c\sim1/L^2$ with the size of the system, and in the thermodynamic limit ($L\rightarrow\infty$) there is no phase transition. For any positive $r$ the system converges to the multicultural state. In this sense, the noise rate $r$ corresponds to temperature $T$.

